Techniques for the calculation of electroweak radiative corrections at the one-loop level and results for W-physics at LEP200

We review the techniques necessary for the calculation of virtual electroweak and soft photonic corrections at the one-loop level. In particular we describe renormalization, calculation of one-loop integrals and evaluation of one-loop Feynman amplitudes. We summarize many explicit results of general relevance. We give the Feynman rules and the explicit form of the counter terms of the electroweak standard model, we list analytical expressions for scalar one-loop integrals and reduction of tensor integrals, we present the decomposition of the invariant matrix element for processes with two external fermions and we give the analytic form of soft photonic corrections. These techniques are applied to physical processes with external W-bosons. We present the full set of analytical formulae and the corresponding numerical results for the decay width of the W-boson and the top quark. We discuss the cross section for the production of W-bosons in e^{+}e^{-}-annihilaton including all O(alpha) radiative corrections and finite width effects. Improved Born approximations for these processes are given.

==> hab9f1.tex <==
\addtocounter{page}{2}
\addtocounter{chapter}{1}
 
\begin{figure}[p]
\savebox{\Vr}(36,0)[bl] 
{\multiput(3,0)(12,0){3}{\oval(6,4)[t]}
\multiput(9,0)(12,0){3}{\oval(6,4)[b]} }
\savebox{\Vt}(0,36)[bl] 
{\multiput(0,3)(0,12){3}{\oval(4,6)[l]}
\multiput(0,9)(0,12){3}{\oval(4,6)[r]} }
\savebox{\Vtr}(36,18)[bl] 
{\multiput(4,0)(8,4){5}{\oval(8,4)[tl]}
\multiput(4,4)(8,4){4}{\oval(8,4)[br]} }
\savebox{\Vbr}(36,18)[bl] 
{\multiput(4,18)(8,-4){5}{\oval(8,4)[bl]}
\multiput(4,14)(8,-4){4}{\oval(8,4)[tr]}}
\savebox{\Vtbr}(36,36)[bl] 
{\put(00,18){\usebox{\Vtr}}
\put(00,00){\usebox{\Vbr}}}
 
\savebox{\Sr}(36,0)[bl] 
{ \multiput(0,0)(13,0){3}{\line(4,0){10}} }
\savebox{\St}(0,36)[bl] 
{ \multiput(0,0)(0,13){3}{\line(0,1){10}} }
\savebox{\Str}(36,18)[bl] 
{ \multiput(0,0)(13,6.5){3}{\line(2,1){10}} }
\savebox{\Sbr}(36,18)[bl] 
{\multiput(0,18)(13,-6.5){3}{\line(2,-1){10}} }
\savebox{\Stbr}(36,36)[bl] 
{\put(00,18){\usebox{\Str}}
\put(00,00){\usebox{\Sbr}}}
 
\savebox{\Fr}(36,0)[bl] 
{ \put(0,0){\vector(1,0){20}} \put(18,0){\line(1,0){18}} }
\savebox{\Ft}(0,36)[bl] 
{ \put(0,0){\vector(0,1){21}} \put(0,18){\line(0,1){18}} }
\savebox{\Ftr}(36,18)[bl] 
{ \put(0,0){\vector(2,1){20}} \put(18,9){\line(2,1){18}} }
\savebox{\Fbr}(36,18)[bl] 
{ \put(36,0){\vector(-2,1){21}} \put(18,9){\line(-2,1){18}} }
\savebox{\Ftbr}(72,72)[bl] 
{\put(00,36){\usebox{\Ftr}}\put(36,54){\usebox{\Ftr}}
 \put(00,18){\usebox{\Fbr}}\put(36,00){\usebox{\Fbr}}}
\savebox{\Vp}(36,36)[bl] 
{ \put(0,18){\circle*{4}} \put(36,0){\circle*{4}} 
\put(36,36){\circle*{4}} }
 
\bma
\barr{l}
\makebox{
%\begin{picture}(108,72)
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$a)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$\gamma,Z$}}
\put(43,54){\makebox(20,10){$f_{i}$}}
\put(43,8){\makebox(20,10){$f'_{j}$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(72,18){\usebox{\Vt}}
\end{picture}}  \\
 
\savebox{\Ftbr}(72,72)[bl] 
{\put(36,18){\usebox{\Ft}}
\put(36,54){\usebox{\Ftr}} \put(36,00){\usebox{\Fbr}}}
 
\makebox{
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$b)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f_{i}$}}
\put(43,54){\makebox(20,10){$\gamma,Z$}}
\put(43,8){\makebox(20,10){$W$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Vtbr}}
\end{picture}}  
\makebox{
\begin{picture}(135,90)
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f'_{j}$}}
\put(43,54){\makebox(20,10){$W$}}
\put(43,8){\makebox(20,10){$\gamma,Z$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Vtbr}}
\end{picture}}  \\
 
\savebox{\Ftbr}(72,72)[bl] 
{\put(00,36){\usebox{\Ftr}}\put(36,54){\usebox{\Ftr}}
 \put(00,18){\usebox{\Fbr}}\put(36,00){\usebox{\Fbr}}}
\makebox{
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$c)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$H,\chi$}}
\put(43,8){\makebox(20,10){$f'_{j}$}}
\put(43,54){\makebox(20,10){$f_{i}$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(72,18){\usebox{\St}}
\end{picture}}  
\\
\savebox{\Ftbr}(72,72)[bl] 
{\put(36,18){\usebox{\Ft}}
\put(36,54){\usebox{\Ftr}} \put(36,00){\usebox{\Fbr}}}
\makebox{
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$d)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f_{i}$}}
\put(43,54){\makebox(20,10){$H$}}
\put(43,8){\makebox(20,10){$W$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Vbr}}
\put(36,36){\usebox{\Str}}
\end{picture}} 
\makebox{
\begin{picture}(135,90)
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f'_{j}$}}
\put(43,54){\makebox(20,10){$W$}}
\put(43,8){\makebox(20,10){$H$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Sbr}}
\put(36,36){\usebox{\Vtr}}
\end{picture}} 
\\
\savebox{\Ftbr}(72,72)[bl] 
{\put(36,18){\usebox{\Ft}}
\put(36,54){\usebox{\Ftr}} \put(36,00){\usebox{\Fbr}}}
\makebox{
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$e)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f_{i}$}}
\put(43,54){\makebox(20,10){$H,\chi$}}
\put(43,8){\makebox(20,10){$\phi$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Stbr}}
\end{picture}} 
\makebox{
\begin{picture}(135,90)
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f'_{j}$}}
\put(43,54){\makebox(20,10){$\phi$}}
\put(43,8){\makebox(20,10){$H,\chi$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Stbr}}
\end{picture}}
\\
\savebox{\Ftbr}(72,72)[bl] 
{\put(36,18){\usebox{\Ft}}
\put(36,54){\usebox{\Ftr}} \put(36,00){\usebox{\Fbr}}}
\makebox{
\begin{picture}(135,90)
\put(-40,60){\makebox(10,10){$f)$}}
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f_{i}$}}
\put(43,54){\makebox(20,10){$\gamma,Z$}}
\put(43,8){\makebox(20,10){$\phi$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Sbr}}
\put(36,36){\usebox{\Vtr}}
\end{picture}} 
\makebox{
\begin{picture}(135,90)
\put(5,40){\makebox(10,10){$W$}}
\put(77,32){\makebox(20,10){$f'_{j}$}}
\put(43,54){\makebox(20,10){$\phi$}}
\put(43,8){\makebox(20,10){$\gamma,Z$}}
\put(100,8){\makebox(10,10){$\bar{f}'_{j}$}}
\put(100,54){\makebox(10,10){$f_{i}$}}
\put(36,18){\usebox{\Vp}}
\put(0,36){\usebox{\Vr}}
\put(36,00){\usebox{\Ftbr}}
\put(36,18){\usebox{\Vbr}}
\put(36,36){\usebox{\Str}}
\end{picture}}
\earr
\ema
\caption{One-loop diagrams for $W \to f_{i}\bar{f}'_{j}$.}
\label{9.1}
\efi
 
\clearpage
 
\addtocounter{page}{-3}
\addtocounter{chapter}{-1}
 
\savebox{\Vr}{}
\savebox{\Vt}{}
\savebox{\Vtr}{}
\savebox{\Vbr}{}
\savebox{\Vtbr}{}
\savebox{\Sr}{}
\savebox{\St}{}
\savebox{\Str}{}
\savebox{\Sbr}{}
\savebox{\Stbr}{}
\savebox{\Fr}{}
\savebox{\Ft}{}
\savebox{\Ftr}{}
\savebox{\Fbr}{}
\savebox{\Ftbr}{}
\savebox{\Vp}{}
 


==> hab9t3.tex <==
\begin{table}
\begin{center}
\begin{tabular}{||r|c|c|c|c||} \hline\hline
\multicolumn{1}{||c|}{$ m_t $} &  $M_H=50 $ &
 $ M_H=100 $ & $ M_H=300 $  & $ M_H=1000 $      \\
 \hline
 80.0 & 0.2212 & 0.2209 & 0.2202 & 0.2193 \\
 \hline
100.0 & 0.2227 & 0.2224 & 0.2217 & 0.2208 \\
 \hline
120.0 & 0.2239 & 0.2236 & 0.2229 & 0.2220 \\
 \hline
140.0 & 0.2251 & 0.2248 & 0.2241 & 0.2232 \\
 \hline
160.0 & 0.2264 & 0.2261 & 0.2254 & 0.2245 \\
 \hline
180.0 & 0.2278 & 0.2276 & 0.2269 & 0.2260 \\
 \hline
200.0 & 0.2294 & 0.2291 & 0.2284 & 0.2275 \\
 \hline\hline
\end{tabular}
\end{center}
\caption{Partial W-decay width $\Gamma^{We\nu}$ including first
order QCD and electroweak corrections for different values of the top 
and Higgs masses.                                                 
All values are given in $\mbox{GeV}$.\label{tab93}}
\end{table}
\begin{table} 
\begin{center}
\begin{tabular}{||r|c|c|c|c||} \hline\hline
\multicolumn{1}{||c|}{$ m_t $} &  $M_H=50 $ &
 $ M_H=100 $ & $ M_H=300 $  & $ M_H=1000 $      \\
 \hline
 80.0 & 0.6539 & 0.6530 & 0.6509 & 0.6481 \\
 \hline
100.0 & 0.6585 & 0.6575 & 0.6554 & 0.6526 \\
 \hline
120.0 & 0.6622 & 0.6612 & 0.6591 & 0.6563 \\
 \hline
140.0 & 0.6659 & 0.6650 & 0.6629 & 0.6601 \\
 \hline
160.0 & 0.6700 & 0.6691 & 0.6670 & 0.6642 \\
 \hline
180.0 & 0.6745 & 0.6736 & 0.6715 & 0.6686 \\
 \hline
200.0 & 0.6793 & 0.6784 & 0.6763 & 0.6735 \\
 \hline\hline
\end{tabular}
\end{center}
\caption{Partial W-decay width $\Gamma^{Wud}$ including first
order QCD and electroweak corrections for different values of the 
top and Higgs masses. All values are given in $\mbox{GeV}$.\label{tab94}}
\end{table}
\begin{table}
\begin{center}
\begin{tabular}{||r|c|c|c|c||} \hline\hline
\multicolumn{1}{||c|}{$ m_t $} &  $M_H=50 $ &
 $ M_H=100 $ & $ M_H=300 $  & $ M_H=1000 $      \\
 \hline
 80.0 & 2.0375 & 2.0347 & 2.0283 & 2.0196 \\
 \hline
100.0 & 2.0517 & 2.0488 & 2.0423 & 2.0336 \\
 \hline
120.0 & 2.0630 & 2.0602 & 2.0537 & 2.0449 \\
 \hline
140.0 & 2.0747 & 2.0719 & 2.0654 & 2.0566 \\
 \hline
160.0 & 2.0872 & 2.0844 & 2.0780 & 2.0692 \\
 \hline
180.0 & 2.1009 & 2.0981 & 2.0917 & 2.0830 \\
 \hline
200.0 & 2.1157 & 2.1129 & 2.1066 & 2.0980 \\
 \hline\hline
\end{tabular}
\end{center}
\caption{Total W-decay width $\Gamma^{W}$ including first
order QCD and electroweak corrections for different values of the 
top and Higgs masses. All values are given in $\mbox{GeV}$.\label{tab95}}
\end{table} 

